Achieving Optimum Received Power with Elementwise Updates in the Least Number of Steps for Discrete-Phase RISs

The problem of optimizing discrete phases in a reconfigurable intelligent surface (RIS) to maximize the received power at a user equipment is addressed. Necessary and sufficient conditions to achieve this maximization are given. These conditions are employed in an algorithm to achieve the maximization. New versions of the algorithm are given that are proven to achieve convergence in N or fewer steps whether the direct link is completely blocked or not, where N is the number of the RIS elements, whereas previously published results achieve this in KN or 2N number of steps where K is the number of discrete phases. Thus, for a discrete-phase RIS, the techniques presented in this paper achieve the optimum received power in the smallest number of steps published in the literature. In addition, in each of those N steps, the techniques presented in this paper determine only one or a small number of phase shifts with a simple elementwise update rule, which result in a substantial reduction of computation time, as compared to the algorithms in the literature. As a secondary result, we define the uniform polar quantization (UPQ) algorithm which is an intuitive quantization algorithm that can approximate the continuous solution with an approximation ratio of sinc^2(1/K) and achieve low time-complexity, given perfect knowledge of the channel.

==> MISOwithKtoInfty.tex <==



\section{MISO with $\kappa \rightarrow \infty$}

In this section, we remark on a special case of a point-to-point downlink multi-input single-output (MISO) communication scenario aided by an RIS, where there is a multi-antenna BS with a single-antenna UE, where the direct BS-UE link is blocked. With this, (\ref{eq:rxSISO}) can be rewritten as
\begin{equation} \label{eq:rxMISO}
    y= {\bf h}_u^H {\bf W} {\bf G} {\bf x} s+z,
\end{equation}
where ${\bf x} \in \mathbb{C}^M$ is the transmit beamforming vector, ${\bf G} \in \mathbb{C}^{N \times M}$ is the equivalent channel of the BS-RIS link, and ${\bf W} = {\rm diag}({\bf w})$. The direct channel from BS to UE and the RIS-UE channels are denoted by ${\bf h}_d \in \mathbb{C}^M$ and ${\bf h}_u \in \mathbb{C}^N$, respectively. 

Taking the far-field regime into account with a physical model that is based on angle directions \cite{MZXWZQ23}, similar to the analysis in \cite{XDMWQ22}, the received signal power in equation (\ref{eq:rxMISO}), i.e., $|y|^2$, can be expressed as
\begin{equation}\label{eq:rxMISOangle}
    |y|^2 = |{\bf bWCx}|^2
\end{equation}
where ${\bf C} = [{\bf a}(\vartheta_{b,1},\varphi_{b,1}), {\bf a}(\vartheta_{b,2},\varphi_{b,2}), \cdots, {\bf a}(\vartheta_{b,M},\varphi_{b,M})]$,
$\mathbf{b}=\mathbf{a}^H(\vartheta_u,\varphi_u)$,
with $\{\vartheta_u, \varphi_u\}$ is the departing direction of the reflected signal 
and $\{\vartheta_{b,m},\varphi_{b,m}\}, m=1,\dots,M$ is the arriving signal direction from BS antenna $m$. Here, ${\bf a}(\vartheta,\varphi)$ is the array response vector defined in (\ref{eq:arrayresp}) in the next section.

Similar to the analysis in the Appendix of \cite{XDMWQ22}, equation (\ref{eq:rxMISOangle}) can be rewritten as
\begin{align}
    |y|^2 &= |{\bf bWCx}|^2 \nonumber \\
    &= {\bf w}^H ({\bf P}^T \odot {\bf R}) {\bf w} \nonumber \\
    &= {\bf w}^H {\bf Q} {\bf w}, \label{eq:MISOpower}
\end{align}
where ${\bf Q} = {\bf P}^T \odot {\bf R}$, ${\bf P} = {\bf Cx} {\bf x}^H {\bf C}^H$, and ${\bf R} = {\bf b}^H {\bf b}$. Since ${\bf Q}$ is a semi-positive definite matrix with rank one, maximizing (\ref{eq:MISOpower}) boils down to maximizing $|{\bf z}^H {\bf w}|$, where ${\bf z}$ is the eigenvector associated with the maximum eigenvalue of ${\bf Q}$. Thus, (P2) must be solved and as addressed in this paper.

==> results.tex <==
%
\section{Results and Remarks}
%


==> statements.tex <==
%%
%\section{Two Statements from \cite{b1}}
%%
\begin{nestedcomment}
Towards achieving its goal, \cite{b1} introduced the following lemma.

{\em Lemma 1:\/} For an optimal solution $(\theta_1^*, \ldots, \theta_n^*)$ to problem (8),
each $\theta_n^*$ must satisfy
\begin{equation}\tag{11}
\theta_n^* = \arg \min_{\theta_n\in \Phi_K} |(\theta_n +\alpha_n - \phase{\mu}) \;{\rm mod}\; 2\pi|
\end{equation}
where $\phase{\mu}$ stands for the phase of $\mu$ in (10)\footnote{To prevent confusion,
we will use the same equation numbers (7)--(13) in \cite{b1}. Our own equation numbers,
not available in \cite{b1}, will begin at (19) and will be incremented from that number
on. Similarly, we will introduce Lemma~2 and Algorithm~2 in lieu of Lemma~1 and Algorithm~1
in \cite{b1}. Note that a lemma or an algorithm with
number 2 does not exist in \cite{b1}.}\footnote{In this paper, we define the ${\rm mod}$
function (the modulus function or the modulo operation) $x\; {\rm mod}\;y$ as the remainder after the
dividend $x>0$ is divided by the divisor $y>0$. We write it as $x\;{\rm mod}\; y$, $x\; (mod\; y)$, or
${\rm mod}\; (x, y)$. For $x<0$ and $y>0,$ we use the convention that the remainder should always
be the smallest such nonnegative number.}.

In \cite{b1}, problem (8) is defined as
\end{nestedcomment}
In this paper, we address the following problem
\begin{align}
\tag{8a}\underset{\mbox{\boldmath$\theta$}}{\rm maximize\ } & f({\mbox{\boldmath$\theta$}})\\
\tag{8b}{\rm subject\ to\ } & \theta_n\in \Phi_K\quad {\rm for}\quad n=1, 2, \ldots, N
\end{align}
where
\begin{equation*}\tag{7b}
f({\mbox{\boldmath$\theta$}}) = \frac{1}{\beta_0^2}\bigg|\beta_0e^{j\alpha_0}+\sum_{n=1}^N \beta_n
e^{j(\alpha_n + \theta_n)}\bigg|^2,
\end{equation*}
$h_n = \beta_ne^{j\alpha_n}$ for $n = 0, 1, \ldots, N$,
and ${\mbox{\boldmath$\theta$}} = (\theta_1, \theta_2, \ldots, \theta_N)$. Also, $g$ is defined as
\begin{equation}\tag{9}
g = h_0 + \sum_{n=1}^N h_n e^{j\theta_n^*}
\end{equation} and $\mu$ as
\begin{equation}\tag{10}
\mu = \frac{g}{|g|}.
\end{equation}

\begin{nestedcomment}
\setcounter{equation}{18}
\begin{comment}
In fact,
\end{comment}
Lemma 1 does not hold. This can be seen by numerical examples. We give one such
example in Table~\ref{tbl:compare}. In this table, we look at the simple case of $K=2$, $N=2$.
According to Lemma 1 in \cite{b1}, the condition in (11) should satisfy (8) for this simple
case. We draw values of $h_n$ according to the first paragraph of Sec.~IV in \cite{b1}. We
list these values in rows 2--4 of Table~\ref{tbl:compare}. We define
\begin{equation}
g_0(\theta_1, \theta_2) = h_0 + \sum_{n=1}^2 h_n e^{j\theta_n}
\end{equation}
and list the values of $g_0(\theta_1,\theta_2)$ for all possible $\theta_1, \theta_2 \in \{0, \pi\}$.
There are four such values and they are listed in rows 5--8 of Table~\ref{tbl:compare}. The
set of values for $\theta_1$ and $\theta_2$ that maximize $|g_0|$, or equivalently, that
achieve $g$ in (9), are $\theta_1 = \theta_2 = \pi$ as in row 8 of Table~\ref{tbl:compare}.
Note that this operation results in $\phase{\mu}=2.3719$ radians as shown in column~5 of
row~8 of Table~\ref{tbl:compare}.

\begin{table*}[!t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
 &${\rm Re}[\cdot]$&${\rm Im}[\cdot]$&$| \cdot |$&$\phase{\cdot}\in [0, 2\pi )$ (rad.)\\
 \hline
 $h_0$& $-2.8267\times 10^{-7}$ & $2.7376\times 10^{-7}$ & $3.9350\times 10^{-7}$ & $2.3722$\\
 $h_1$& $1.0958\times 10^{-10}$ & $-1.0501\times 10^{-11}$ & $1.1008\times 10^{-10}$ & $6.1876$\\
 $h_2$& $-1.2238\times 10^{-11}$ & $-2.6605\times 10^{-11}$ & $2.6634\times 10^{-10}$ & $4.6664$\\
 \hline
 $g_0(\theta_1=0,\theta_2=0)$&$-2.8257\times 10^{-7}$&$2.7348\times 10^{-7}$&$3.9324\times 10^{-7}$&$2.3725$\\
 $g_0(\theta_1=0,\theta_2=\pi)$&$-2.8255\times 10^{-7}$&$2.7401\times 10^{-7}$&$3.9359\times 10^{-7}$&$2.3715$\\
 $g_0(\theta_1=\pi,\theta_2=0)$&$-2.8279\times 10^{-7}$&$2.7350\times 10^{-7}$&$3.9341\times 10^{-7}$&$2.3729$\\
 $g_0(\theta_1=\pi,\theta_2=\pi)$&$-2.8277\times 10^{-7}$&$2.7403\times 10^{-7}$&${\bf 3.9377}\times {\bf 10^{-7}}$&$\bf 2.3719$\\
 \hline
\end{tabular}
\caption{Sample calculation for attempting to find optimum $\theta_1^*, \theta_2^*,\ldots,\theta_N^*$ to maximize $|g_0|$ where $g_0 (\theta_1, \theta_2, \ldots, \theta_N) = h_0 + \sum_{n=1}^N h_n e^{j\theta_n}$ with $\theta_n\in\Phi_K = \{0,\frac{2\pi}{K},\ldots,(K-1)\frac{2\pi}{K}\}$, $n=1, 2, \ldots, N$, for $K=2$ and $N=2$. Channel coefficients $h_n$, $n=0,1,2$ are calculated using the technique described in \cite{b1}.
Rows 5--8 present all values of $g_0$ with all combinations of $\theta_1, \theta_2 \in \Phi_2$, showing that $|g| = \max |g_0 (\theta_1, \theta_2) |$ is achieved with $\theta_1^* =\theta_2^* = \pi$.
}
\label{tbl:compare}
\end{center}
\end{table*}
\begin{table}[!t]
\begin{center}
\begin{tabular}{|c|c|}
\hline
$(\theta_1=0)+\alpha_1-\phase{\mu}$&{3.8158}\\
${\rm mod} ((\theta_1=0)+\alpha_1-\phase{\mu},2\pi)$&{3.8158}\\
$(\theta_1=\pi)+\alpha_1-\phase{\mu}$&{6.9574}\\
${\rm mod} ((\theta_1=\pi)+\alpha_1-\phase{\mu},2\pi)$&{\bf 0.67417}\\[0.7mm]
 \hline
$(\theta_2=0)+\alpha_2-\phase{\mu}$&{2.2945}\\
${\rm mod} ((\theta_2=0)+\alpha_2-\phase{\mu},2\pi)$&{\bf 2.2945}\\
$(\theta_2=\pi)+\alpha_2-\phase{\mu}$&{5.4361}\\
${\rm mod} ((\theta_2=\pi)+\alpha_2-\phase{\mu},2\pi)$&{5.4361}\\[0.7mm]
 \hline
$\cos((\theta_1=0)+\alpha_1-\phase{\mu})$&{-0.7812}\\
$\cos((\theta_1=\pi)+\alpha_1-\phase{\mu})$&{\bf 0.7812}\\[0.7mm]
 \hline
$\cos((\theta_2=0)+\alpha_2-\phase{\mu})$&{-0.6672}\\
$\cos((\theta_2=\pi)+\alpha_2-\phase{\mu})$&{\bf 0.6672}\\[0.7mm]
\hline
\end{tabular}
\caption{Continuation of the sample calculation for attempting to find optimum $\theta_1^*, \theta_2^*,\ldots,\theta_N^*$ to maximize $|g_0|$. Rows 1--8 present the calculation of $\min_{\theta_n\in \Phi_K} \;{\rm mod}\; (\theta_n + \alpha_n - \phase{\mu}, 2\pi)$ for $n=1,2,\ldots,N$, as specified in \cite{b1} to attempt to find the optimum values of $\theta_n$. This calculation results in values $\theta_1=0$ and $\theta_2=\pi$, which are not $\theta_1^*, \theta_2^*$. Rows 9-12 present the calculation of $\max_{\theta_n\in \Phi_K} \cos(\theta_n + \alpha_n - \phase{\mu})$ to find $\theta_1^*, \theta_2^*, \ldots, \theta_N^*$ as discussed in this comment. This technique finds the optimum values of $\theta_n,$ $n=1,2,\ldots, N$.
}
\label{tbl:compare2}
\end{center}
\end{table}
At this point, we would like to emphasize that \cite{b1} uses a particular convention for the
phases of complex numbers. They are defined to be in $[0, 2\pi)$, see the text that follows
(2) in \cite{b1}. We use the same convention in generating Table~\ref{tbl:compare}, see its
column 5, as well as in generating Table~\ref{tbl:compare2}. With this convention, we list
 $\theta_n + \alpha_n -\phase{\mu}$ and
$(\theta_n + \alpha_n - \phase{\mu}) \;{\rm mod}\; 2\pi$ for possibilities of $\theta_n = 0$ and
$\theta_n=\pi$ and
$n=1,2$ in rows 1--8 of Table~\ref{tbl:compare2}.\footnote{Note that absolute value
signs in (11) are not needed since the argument of the minimum operation
in (11) is in $[0, 2\pi)$.} It can be seen from rows~1--4 of Table~\ref{tbl:compare2}
that the method results in $\theta_1 = \pi$ as the potential $\theta_1^*$, which we
know from the discussion in the previous paragraph to be correct. When we carry out
the calculation $(\theta_2 + \alpha_2 - \phase{\mu}) \; {\rm mod}\; 2\pi$ in rows 5--8 of
Table~\ref{tbl:compare2}, we find that the method suggests $\theta_2=0$ should be
$\theta_2^*$. However, we know from the exhaustive search in rows 5--8 of
Table~\ref{tbl:compare} that $\theta_2^*=\pi$. Thus, Lemma~1 is not correct.
\end{nestedcomment}
It is possible to come up with a correct lemma similar to Lemma~1. We
specify this lemma below.

{\em Lemma 2:\/} For an optimal solution $(\theta_1^*, \theta_2^*, \ldots,
\theta_n^*)$, it is necessary and sufficient that each $\theta_n^*$ satisfy
\begin{equation}
\theta_n^* = \arg \max_{\theta_n\in \Phi_K} \cos(\theta_n + \alpha_n -\phase{\mu})
\label{eqn:lemma2}
\end{equation}
where $\phase{\mu}$ stands for the phase of $\mu$ in (10).

{\em Proof:\/} We can rewrite (9) as
\begin{align}
|g| =& \ \beta_0 e^{j(\alpha_0-\phase{\mu})} + \sum_{n=1}^N \beta_n e^{j(\alpha_n+\theta_n-\phase{\mu})} \\
 = & \ \beta_0 \cos(\alpha_0 - \phase{\mu}) + j \beta_0 \sin (\alpha_0-\phase{\mu}) \nonumber\\
 & + \sum_{n=1}^N \beta_n \cos(\theta_n + \alpha_n - \phase{\mu}) \nonumber\\
 & + j \sum_{n=1}^N \beta_n \sin(\theta_n + \alpha_n - \phase{\mu}).
 \label{eqn:absg}
\end{align}
Because $|g|$ is real-valued, the second and fourth terms in (\ref{eqn:absg}) sum to zero, and
\begin{equation}
|g| = \beta_0 \cos(\alpha_0 - \phase{\mu}) + \sum_{n=1}^N \beta_n \cos(\theta_n + \alpha_n - \phase{\mu})
\end{equation}
from which (\ref{eqn:lemma2}) follows as a necessary and sufficient condition for Lemma~2 to hold.
\hfill$\blacksquare$

Rows~9--12 of Table~\ref{tbl:compare2} illustrate that this method finds $\theta_1^*$ and $\theta_2^*$.
More extensive calculations can be carried out to show that an exhaustive search as in rows 5--8 of
Table~\ref{tbl:compare} confirms that Lemma~2 holds for a wide set of $K$ and $N$ values as well as
a wide set of channel coefficients $h_0, h_1, \ldots, h_N$.

Reference \cite{b1} attempts to decide a range of $\mu$ for which $\theta_n^* = k\omega$ must hold,
making use of Lemma~1. Towards that end, it first defines a sequence of complex numbers with respect to
each $n=1,2,\ldots,N$ as
\begin{equation}\tag{12}
s_{nk} = e^{j(\alpha_n+(k-0.5)\omega)},\ {\rm for}\ k=1,2,\ldots,K.
\label{eqn:eqn12}
\end{equation}
Then, \cite{b1} defines, for any two points $a$ and $b$ on the unit circle $C$, ${\rm arc}(a:b)$
to be the unit circular arc with $a$ as the initial end and $b$ as the terminal end in the counterclockwise
direction; in particular, it defines ${\rm arc}(a:b)$ as an open arc with the two endpoints $a$ and $b$
excluded. With this definition, \cite{b1} states the following proposition follows from Lemma 1.

{\em Proposition 1:\/} A sufficient condition for $\theta_n^*=k\omega$ is
\begin{equation}\tag{13}
\mu \in {\rm arc} (s_{nk}:s_{n,k+1}).
\end{equation}
Reference \cite{b1} states that ``letting $\theta_n = k\omega$ is guaranteed to minimize the gap
$|(\theta_n+\alpha_n-\phase{\mu}) \;{\rm mod}\; 2\pi |$ whenever $\mu$ lies in its associated arc, and thus
$k\omega$ must be optimal according to Lemma 1.''

Now, let $K=2$ and thus $\omega=\frac{2\pi}{K}=\pi$, and the two possibilities for $\theta$ are
$\theta^1=\pi$ and $\theta^2 = 2\pi$, or equivalently $\theta^2 = 0$. According to (12), we have
\begin{equation}
s_{n1}=e^{j(\alpha_n+\frac{\pi}{2})},\quad s_{n2}=e^{j(\alpha_n+\frac{3\pi}{2})}.
\end{equation}
According to Proposition~1, if $\mu\in {\rm arc}(s_{n1}:s_{n2})$ then $\theta_n^*=\omega=\pi$
should hold. Assume $\mu$ is in ${\rm arc}(s_{n1},s_{n2})$. Then, it can be observed that
$\alpha_n-\phase{\mu}\in (\frac{\pi}{2},\frac{3\pi}{2})$, paying
attention to the change of order due to the subtraction of $\phase{\mu}$. In particular, let
$\mu$ be
such that $\alpha_n-\phase{\mu}\in (\frac{\pi}{2},\pi)$. When this is the case, note that $(\theta^1
+\alpha_n - \phase{\mu})\in (\frac{3\pi}{2}, 2\pi)$ while $(\theta^2+\alpha_n-\phase{\mu})\in
(\frac{\pi}{2},\pi)$. Thus, $|(\theta^2 + \alpha_n - \phase{\mu}) \;{\rm mod}\; 2\pi| <
|(\theta^1 + \alpha_n - \phase{\mu}) \;{\rm mod}\; 2\pi|$, and according to Lemma~1,
$\theta_n^*=\theta^2=0$, in contradiction with Proposition~1.
On the other hand, Proposition~1 is compatible with Lemma~2. To see this, assume
$\mu$ satisfies (12). Then,
\begin{equation}
\phase{\mu}\in \Big(\alpha_n+\Big(k-\frac{1}{2}\Big)\omega,\alpha_n+\Big(k+\frac{1}{2}\Big)\omega\Big).
\end{equation}
Since $\omega=\frac{2\pi}{K}$,
\begin{equation}
\alpha_n-\phase{\mu}\in \Big((-2k-1)\frac{\pi}{K}, (-2k+1)\frac{\pi}{K}\Big)
\end{equation}
considering the reversal of order due to the substraction of $\phase{\mu}$.
Now, let $\theta_n = k\omega = 2k \frac{\pi}{K}$. Then
\begin{equation}
\theta_n + \alpha_n - \phase{\mu} \in \Big(-\frac{\pi}{K}, \frac{\pi}{K}\Big)
\end{equation}
and thus $\cos(\theta_n + \alpha_n-\phase{\mu})$ is the largest among
all other possibilities for $\theta_n$ because the slice $(-\frac{\pi}{K}, \frac{\pi}{K})$ corresponds
to the largest values of the cosine function among all slices corresponding to different values of
$\theta_k \in \Phi_K$ for $k=1,2,\ldots,K$.



